Learning to guide task and motion planning using score-space representation

In this paper, we propose a learning algorithm that speeds up the search in task and motion planning problems. Our algorithm proposes solutions to three different challenges that arise in learning to improve planning efficiency: what to predict, how to represent a planning problem instance, and how to transfer knowledge from one problem instance to another. We propose a method that predicts constraints on the search space based on a generic representation of a planning problem instance, called score-space, where we represent a problem instance in terms of the performance of a set of solutions attempted so far. Using this representation, we transfer knowledge, in the form of constraints, from previous problems based on the similarity in score space. We design a sequential algorithm that efficiently predicts these constraints, and evaluate it in three different challenging task and motion planning problems. Results indicate that our approach performs orders of magnitudes faster than an unguided planner

==> intro_arvix.tex <==
\section{1. Introduction}

Task and motion planning (TAMP) problems are sequential
decision making problems in which a robot is required to
search for a sequence of decisions that account for both
discrete and continuous aspects of the world to achieve 
a high-level goal. These decisions are intricately related to
one another, and they must abide by collision-constraints and
transition dynamics.

 A variety of planners have been developed
for TAMP problems~\citep{GravotISRR05,TLPKBel13,TLPIROS14,SrivastavaICRA14,
ToussaintIJCAI15,DantamRSS17}.
However, their worst-case computation time generally scales
exponentially with problem size, and each new problem instance must be
solved from scratch, making them inefficient for real-world tasks.
 In contrast, humans are able to short-cut their
planning process by learning to adapt previous planning experience to
reduce the search space intelligently for new problem instances.
This observation motivates the design of an algorithm that learns from
experience to make predictions that guide the search of a
planner.  We face three important questions in designing the learning
algorithm: (1) what to predict, (2) how to represent a problem
instance, and (3) how to transfer knowledge from past experience to
the current problem instance.


\begin{figure}
\centering
\includegraphics[height=4.5cm,width=4.2cm]{./figures/motiv_metric2_.png}
\includegraphics[height=4.5cm,width=4.2cm]{./figures/motiv_metric1_.png}\\
\caption{The task is to pick up the blue object by planning a collision-free path from an
 initial configuration to a pre-grasp configuration. When the obstacle (pink cup) moves 
even by 0.02m, this requires a qualitatively different collision-free path.}
\label{fig:motiv2}
\end{figure} 



The first challenge is what to predict.  Previous approaches to using
learning to speed up planning have tried predicting a complete solution,
or a subgoal that fully specifies the robot configuration and world state,
including object poses. However, because of the intricate 
relationship between object poses and the robot's free-space, a small
change in the environment may completely alter the space of feasible
solutions.  This lack of regularity in the relationship between a problem
instance and its solution makes it difficult to predict a complete
solution or a subgoal based on experience. This difficulty is 
illustrated in Figure~\ref{fig:motiv2} in a pick domain.


\begin{figure}
\centering
\includegraphics[scale=0.2]{./figures/choosing_grasp1}
\includegraphics[scale=0.2]{./figures/choosing_grasp2}
\caption{Two instances of the grasp selection domain. The arrangement and number of
  obstacles vary randomly across different planning problem instances. The objective
is to find an arm trajectory to a pre-grasp pose for the blue box, marked with a circle, whose pose
is randomly determined in each problem instance}
\label{fig:grasp_domain}
\end{figure}


Building on this observation, we instead learn to predict
constraints on the solution by finding a subset of decision
variables that can be predicted reliably, while
 leaving the rest of the decision variables to be
filled in by the planner. This decomposition is based on the intuition
that constraints can generalize more effectively across problem
instances than a complete solution or a subgoal. For instance,
consider a robot trying to pick an object from a shelf, as shown in
Figure \ref{fig:grasp_domain} (right). A constraint that forces
the robot to approach the object either from the side or the top, depending 
on whether the object is on the table or the shelf, can be used more reliably 
across different arrangements of obstacles and object poses than a detailed 
path plan or a specific pre-grasp configuration.


We will refer to the subset of decision variables that we predict as
\emph{solution constraints}, or constraints for short.  
Solution constraints, when intelligently
chosen, will effectively reduce the search space while preserving the
robustness of the planner against changes in problem instances. 

These points are illustrated in Figure~\ref{fig:constraint_illustration}.
Notice how the reduced search space that satisfies the given constraint
is much smaller than the original search space. 
The planner now only has to find a solution within this space,
requiring much less computation than the unconstrained planner.
Also notice that unlike a complete plan, a constraint is more
general in the sense that a single constraint can be applied to
a set of problems instead of a single problem.

\begin{figure}
\centering
\includegraphics[scale=0.3]{./figures/constraint_illustration}
\caption{A comparison of search done by a planner
without a constraint, and with constraint that forces
the planner to find a solution that approaches the target object from
the top. The black arrow indicates the work done by a machine learning algorithm,
which predicts a constraint, and the yellow arrow indicates 
the work done by a constrained planner.
The gray blob in the space of plans show the reduced search space
that satisfies the constraint. The yellow blob in the space of
problems indicate the set of problem instances for which
there exists a plan that satisfies the top-grasp constraint. 
The yellow star indicates the given problem instance.}
\label{fig:constraint_illustration}
\end{figure}

The second challenge is representing problem instances. In most
of the TAMP problems that we are contemplating, a manual design of 
a generic feature representation for predicting constraints is difficult: there are 
varying numbers and shapes of objects for each problem instance, 
and some object relations matter for some problem instances but
not for others. For instance, in Figure \ref{fig:grasp_domain} (left),
the obstacles on the desk influence how the robot
should pick the blue object and the obstacles on the shelf are
irrelevant. On the other hand, in Figure  \ref{fig:grasp_domain} (right),
the obstacles on the desk are irrelevant.

In light of this, we propose a new type of representation for problem
instances, called \emph{score-space}. In a score-space representation,
 we represent a problem instance
in terms of a vector of the scores for a set of plans on that
instance, where each of the plans is computed based on one of a fixed
set of promising solution constraints. The intuition is that what matters in a 
planning problem is how an environment responds to a potential solution, and a 
good way to predict what solution constraints will work well is to consider
how effective other solution constraints have been. 
Figure~\ref{fig:score_space_illustration}
shows examples of score-space representations of different 
TAMP problem instances. 
\begin{figure}
\centering
\includegraphics[scale=0.3]{./figures/score_space_illustration}
\caption{An illustration of a score-space representation of
three different problem instances. We assume an one-dimensional 
constraint for the illustration purpose. The x-axis of
a score function represents different values of constraints,
and y-axis represents the score of a plan that conforms to a 
constraint.}
\label{fig:score_space_illustration}
\end{figure}

  The main advantage of the score-space representation
is that it gives direct information about similarity between problem instances and 
solution constraints, without depending on a hand-designed representation.
Similar problem instances will have similar patterns of scores on different
constraints, and similar constraints will have similar patterns of scores
on different problem instances.


 For instance, consider again the task in Figure \ref{fig:grasp_domain}. 
By computing a plan associated
with the solution constraint that forces the robot to  approach the 
object from the top and
observing that it has a low score, we can learn that it is occluded from
above, e.g. by a shelf, and can predict other more appropriate action choices.
This information is not biased by the designer's choice of representation: having
learned that approaching the object from the side did not work,
a learning algorithm may try to approach the object from the top. Such reasoning
is much more difficult when the learning algorithm is forced
to reason in terms of a particular representation of the problem,
such as poses of obstacles or 2D or 3D images of the scene. 
The main disadvantage is that the score-space information is
computationally expensive to obtain, since it requires computing
the plans associated with solution constraints.

This observation brings us to the third challenge of
 learning to plan, which is how to transfer knowledge from past experience
to the current problem instance efficiently.  We propose to solve this challenge
by using the expectation and correlation of the scores of solution
constraints from past problem instances to determine which solution
constraint to try next. Our intuition is that the solution constraints
that performed well or poorly together are more likely to do so in a
new problem instance; for instance, in the previous example for
picking an object from a shelf, grasps from the sides would have worked
well in most of the problem instances, while grasps from the top or bottom
would have worked poorly.

Building on this intuition, we propose an algorithm that directly
reasons with the correlation information in the score-space 
representation of a problem instance. We
assume that a score vector that represents a problem instance is
distributed according to a Gaussian distribution, 
and propose~\boxalg, which is an upper-confidence-bound (UCB)
type, experience-based, black-box function-optimization
technique~\citep{MunosFTML14,SrinivasICML10}.~\boxalg~learns 
to suggests solution constraints based on its belief
about the scores of solution constraints, whose prior
distribution is computed using scores of constraints
in the past planning problem instances, and whose 
posterior distribution is defined by updating the parameters
of the Gaussian distribution using the score feedback from the environment.

\iffalse
The overall work-flow is shown in Figure~\ref{fig:box_overall}.
 
\begin{figure*}
\centering
\includegraphics[scale=0.35]{./figures/box_overall}
\caption{Overall work-flow of BOX. It receives prior experience data
in the form of score values, which it uses to compute the prior belief
of scores of a current problem instance. It then suggests a constraint 
to the current problem instance, receives a score, and updates its
belief. This process is repeated until we find a solution.} 
\label{fig:box_overall}
\end{figure*}
\fi

This paper is an improved and extended version of our prior paper~\citep{KimICRA17}.
In particular, we make the following additional contributions. 
\begin{itemize}
\item We prove that our algorithm has a sublinear regret in number
of evaluations under
certain conditions, using the theoretical results from
Bayesian optimization literature~\citep{SrinivasICML10}. 
\item We propose a new algorithm 
that reduces the cardinality of an initial set of constraints. 
It reduces the worst-case evaluation time, the computation
time for updating the covariance matrix, and the number of
evaluations of a constraint. We add experiments to evaluate
the effect of this algorithm. 
\item We present a new simulation result that requires a significantly
longer planning horizon than the ones that we considered
in our prior work. Besides the longer horizon, this new
domain is especially hard because uniform random sampling
of actions would
frequently call a motion planner on infeasible problem 
instances. 
\end{itemize}

In all of the tasks, we show that~\boxalg~can accelerate planning 
significantly over a basic planner that does not use solution
constraints.  We also provide a comparison to a sampler that picks
solution constraints uniformly at random, and to a state-of-the-art black-box
function optimization technique called deterministic optimistic
optimization (DOO)~\citep{MunosNIPS11} that does not use the score space
representation. We find that~\boxalg~ outperforms these other methods.
Additional experiments on using a minimal constraint set built
using our greedy algorithm indicate that
we can almost completely eliminate the covariance matrix
inversion time for~\boxalg, and reduce the total planning time by
a factor of 5 for some domains.







